Facade-X: an opinionated approach to SPARQL anything

The Semantic Web research community understood since its beginning how crucial it is to equip practitioners with methods to transform non-RDF resources into RDF. Proposals focus on either engineering content transformations or accessing non-RDF resources with SPARQL. Existing solutions require users to learn specific mapping languages (e.g. RML), to know how to query and manipulate a variety of source formats (e.g. XPATH, JSON-Path), or to combine multiple languages (e.g. SPARQL Generate). In this paper, we explore an alternative solution and contribute a general-purpose meta-model for converting non-RDF resources into RDF: Facade-X. Our approach can be implemented by overriding the SERVICE operator and does not require to extend the SPARQL syntax. We compare our approach with the state of art methods RML and SPARQL Generate and show how our solution has lower learning demands and cognitive complexity, and it is cheaper to implement and maintain, while having comparable extensibility and efficiency.

==> sections/related-work-extended.tex <==
We place our research in the area of semantic web approaches to content re-engineering.
Related work includes also approaches to extending the functionalities of the SPARQL query language.
Finally, research on end-user development and human interaction with data gives a background to our contribution.

The Semantic Web research community understood since its beginning how crucial it is to equip practitioners with flexible and usable methods to transform non-RDF resources into RDF. 

In the literature on ontology engineering, non-ontological resource re-engineering refers to the process of taking an existing resource and transforms it into an ontology. A classification of types of sources for ontology engineering is proposed in~\cite{villazon2010pattern}, where non-ontological resource formats are classified as XML, flat files, relational databases, and spreadsheets. The proposed approach is based on a set of intermediate abstract data models mainly targeted to re-engineering classification schemes. 
These family of approaches are based on the assumption that there is a known target ontology to be used as a reference model for transforming both schema and data. Therefore, it cannot be applied to the case of re-engineering content to RDF \textit{in absence} of a specific domain model.

Triplify~\cite{auer2009triplify} is one of the first tools aiming at converting sources into RDF in a domain independent way. The approach is based on mapping HTTP URIs to ad-hoc database queries, and rewriting the output of the SQL query into RDF. The output RDF is generated by mapping table columns to RDF properties and cell values to RDF literals. However, setting up a Triplify endpoint requires deep knowledge of the underlying relational database model for preparing accurate transformations.
From the perspective taken in the present work, the problem of re-engineering relational databases into RDF can be considered solved by the W3C Direct Mapping recommendation~\cite{w3c:directmapping}, and we don't discuss it further.
% \paragraph{Approaches to reengineering}
% GRDDL, XSPARQL, R2RML, RML~\cite{dimou2014rml}, CSVW, ...

A long history of mapping languages for transforming heterogeneous files into RDF can be considered superseded by RML~\cite{dimou2014rml}, also specialised to support data cleaning operations~\cite{slepicka2015kr2rml} and specific forms of data, for example, relational~\cite{rodriguez2015efficient} or geospatial data~\cite{kyzirakos2014geotriples}.
This family of solutions are based on a set of declarative rules that Semantic Web practitioners are expected to develop by analysing the input data sources. 
The language allows to embed format-specific query languages (e.g. XPath) and require the practitioner to have deep knowledge not only of the input data model but also of standard methods used for its processing.
Recent work acknowledges how these languages are built with machine-processability in mind~\cite{heyvaert2018declarative} and how defining or even understanding the rules is not trivial to users.

We survey approaches to extend SPARQL. A standard method for extending SPARQL is by providing custom functions to be used in FILTER or BIND operators. ARQ provides a library of custom functions for supporting aggregates such as computing a standard deviation of a collection of valyes\footnote{ARQ functions: \url{https://jena.apache.org/documentation/query/extension.html} (accessed 15/12/2020).}
Query processing engines can extend SPARQL by using so-called magic properties. This approach defines custom predicates to be used for instructing specific behavior at query execution. For example, this allows the specification of complex fulltext searches over literal values. Query processors can delegate execution to a fulltext engine (e.g. Lucene) and return a collection of query solutions as triple patterns. % A similar approach can be used to support XPATH, XQuery in Virtuoso, which also allows to embed SQL functions in SPARQL to query directly the underlying relational model\footnote{Virtuoso Open Source. SPARQL inline in SQL: \url{http://docs.openlinksw.com/virtuoso/rdfsparqlinline/}.}. 

SPARQL Generate~\cite{lefranccois2017sparql} introduces a novel approach for performing data transformation from heterogeneous sources into RDF by extending the SPARQL syntax with a new GENERATE operator~\cite{lefranccois2017sparql}. 
The method introduces two more operators, SOURCE and ITERATOR.
Custom functions perform ad-hoc operations on the supported formats, for example, relying on XPath or JSONPath.
However, using SPARQL Generate require users to have knowledge of the source formats and of the toolset available to manipulate them, often including external specifications (such as XPath).
In addition, implementing the SPARQL Generate approach requires implementing a new syntax parser which violates the SPARQL 1.1 standard syntax.

However, there are approaches to extend SPARQL without changes to the standard syntax.
For example,~\cite{daga2015basilar} allows to define parametric queries by enforcing a convention in SPARQL variable names. As a result, SPARQL query templates can be processed with standard query parsers.
In this paper, we follow a similar, minimalist approach and extend SPARQL by \textit{overriding} the behaviour of the SERVICE operator. % and define a custom URI-schema that can be used as a (virtual) endpoint URL\footnote{URI Schemas on Wikipedia: \url{https://en.wikipedia.org/wiki/List\_of\_URI\_schemes} (accessed 15/12/2020).}.
Later, we will compare our proposal with SPARQL Generate and RML in detail.

%
% Querying APIs with SPARQL
% https://www.sciencedirect.com/science/article/abs/pii/S0306437920301125
%
% Read https://link.springer.com/chapter/10.1007/978-3-030-50439-7_4
%

Motivation for our work resides in research on end-user development and human interaction with data.
End-user development is defined by~\cite{lieberman2006end} as "methods, techniques, and tools that allow users of software systems, who are acting as non-professional software developers, at some point to create, modify or extend a software artefact."  Many end-user development tasks are concerned with the use of software to manipulate data. End-user development initially focused on the use of spreadsheets and related tools to support the manipulation of data on desktop computers, and has since expanded to encompass end-users programmatically sending, receiving and manipulating data from web APIs, IoT devices and robots \cite{paterno2019end}.

Unlike professional software development, end-user development involves the construction of software for personal rather that public use \cite{ko2011state} in order to carry out professional activities. Many SPARQL users fall into the category of end-user developer. \cite{warren2018using} in a survey of SPARQL users, found that although 58\% came from the computer science and IT domain, other SPARQL users came from areas including social sciences and humanities, business and economics, and biomedical, engineering or physical sciences.

Although spreadsheets have become the most ubiquitous end-user development tool, their use can be error prone \cite{panko2010revising}, for example, selecting the wrong cell or region of cells in a formula.  Although some errors are due to human slips and interface usability problems, others are due to the 2D tabular nature of the spreadsheet not adequately reflecting the data structures with which the user is trying to work. The data with which users work is often primarily list-based and/or hierarchical rather than tabular. \cite{miller2016gradual} developed an extension to the spreadsheet in which a formula can explicitly reference a list (e.g. a column of numbers) rather than the formula being copied to every cell in the column of a table. \cite{chang2016using} propose an extension to spreadsheets to explicitly support hierarchical data, through the nesting of cells, for example cell B1.1 being a sub-cell of B1. \cite{hall2019lish} proposes an alternative formulation to spreadsheets in which data is represented as nested lists, rather than tables. This has a number of potential advantages over the conventional spreadsheet. First, it provides a meaningful level of abstraction in which a set of related cells (e.g a table column) can be treated as a first class object. Second, it supports a more exploratory way of working in which data does not have to be prematurely fitted into a 2D grid structure, which may later be found to be not fit for purpose. Third, it offers greater support for reuse; functions for manipulating list-based and hierarchical structures can be reused across different datasets without the error-prone copying, pasting and editing of formulae.
